A Machine Learning and Computer Vision Approach to Geomagnetic Storm Forecasting

Geomagnetic storms, disturbances of Earth's magnetosphere caused by masses of charged particles being emitted from the Sun, are an uncontrollable threat to modern technology. Notably, they have the potential to damage satellites and cause instability in power grids on Earth, among other disasters. They result from high sun activity, which are induced from cool areas on the Sun known as sunspots. Forecasting the storms to prevent disasters requires an understanding of how and when they will occur. However, current prediction methods at the National Oceanic and Atmospheric Administration (NOAA) are limited in that they depend on expensive solar wind spacecraft and a global-scale magnetometer sensor network. In this paper, we introduce a novel machine learning and computer vision approach to accurately forecast geomagnetic storms without the need of such costly physical measurements. Our approach extracts features from images of the Sun to establish correlations between sunspots and geomagnetic storm classification and is competitive with NOAA's predictions. Indeed, our prediction achieves a 76% storm classification accuracy. This paper serves as an existence proof that machine learning and computer vision techniques provide an effective means for augmenting and improving existing geomagnetic storm forecasting methods.

==> ongeomagneticstorms.tex <==
Emergency and disaster risk services such as weather forecasting, geo-positioning, and telecommunication heavily rely on their communications with orbital satellites. Current methods of forecasting geomagnetic storms rely on data from solar wind measurement spacecraft in orbit, and magnetometer measurements at physical locations across the world.

\subsection{Technological Vulnerabilities}
Geomagnetic storms can interfere with the functionality of satellites and the power grid. For example, an extreme geomagnetic storm can present an array of effects on satellites, the most important being orientation issues. A storm of this magnitude can create lot's of satellite drag; reducing the speed of the satellite and ultimately decreasing the satellites lifetime as a result. Not only do we lose satellite connections, but also add to the growing problem of space junk in orbit around Earth. On ground level, an extreme storm case can cause widespread voltage control problems and some power grid systems can experience complete collapse \cite{noauthor_noaa_nodate}.

\subsection{Prediction Methods}
The SWPC at NOAA currently has methods to forecast the Kp-Index for the next 3 days, and issue warnings when the Kp-Index value is expected to be greater than or equal to 5. According to the SWPC, methods to predict and estimate the Kp-Index require a collection of ground-based magnetometer measurements from stations around the world, and real-time solar wind measurements from a network of orbital spacecraft \cite{noauthor_3-day_nodate}. Magnetometers measure the magnetic field strength in a particular area, and measurements taken from each station is compiled into the global average Kp-Index. Orbital spacecraft and magnetometer stations used to collect data is not only expensive, but can be unreliable and inefficient. The current state of ground-based magnetometers are quickly aging and becoming a liability \cite{engebretson_future_2017}.

In our approach, we introduce forecasting geomagnetic storms from visual, active sunspot features extracted by computer vision. Those features can then be exploited by machine learning to accurately forecast these storms. Our approach requires nothing but an image of the Sun from a single satellite, forgoing the need of a solar wind spacecraft network and magnetometer stations. Machine learning and computer vision has been proven to be a valuable option when it comes to making intelligent inferences when given non-numerical data.
